Metastability-Containing Circuits

In digital circuits, metastability can cause deteriorated signals that neither are logical 0 or logical 1, breaking the abstraction of Boolean logic. Unfortunately, any way of reading a signal from an unsynchronized clock domain or performing an analog-to-digital conversion incurs the risk of a metastable upset; no digital circuit can deterministically avoid, resolve, or detect metastability (Marino, 1981). Synchronizers, the only traditional countermeasure, exponentially decrease the odds of maintained metastability over time. Trading synchronization delay for an increased probability to resolve metastability to logical 0 or 1, they do not guarantee success. We propose a fundamentally different approach: It is possible to contain metastability by fine-grained logical masking so that it cannot infect the entire circuit. This technique guarantees a limited degree of metastability in---and uncertainty about---the output. At the heart of our approach lies a time- and value-discrete model for metastability in synchronous clocked digital circuits. Metastability is propagated in a worst-case fashion, allowing to derive deterministic guarantees, without and unlike synchronizers. The proposed model permits positive results and passes the test of reproducing Marino's impossibility results. We fully classify which functions can be computed by circuits with standard registers. Regarding masking registers, we show that they become computationally strictly more powerful with each clock cycle, resulting in a non-trivial hierarchy of computable functions.

==> tikzlibrarycircuits.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
%  pgflibrarytikzcircuits.code.tex                                   %
%                                                                    %
%  Version 0.0.1                                                     %
%                                                                    %
%  Authors: Juergen Werber and Christoph Bartoschek                  %
%  Email:   bartoschek -at- or.uni-bonn.de                           %
%                                                                    %
% This file may be distributed and/or modified                       %
%   1. under the LaTeX Project Public License Version 1.3 or later   %
% and/or                                                             %
%   2. under the GNU Public License Version 2 or later.              %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%   USAGE EXAMPLE   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \documentclass{article}
% \usepackage{tikz}
% \usetikzlibrary{circuits}
%
% \begin{document}
% \begin{tikzpicture}[scale=0.5,cktbaselength=0.5pt]
% \draw (6,0) node[nand2ni,anchor=tip,draw] (n4) {}
%       (n4.z) -- +(0mm,-5mm)
%       (n4.b) |- ++(10mm,2mm) -- ++(0mm,2mm)
%       node[and2in,anchor=z,draw,fill=gray] (n3) {}
%       (n4.a) |- ++(-10mm,2mm) -- ++(0mm,2mm)
%       node[or3nni,anchor=tip,draw] (n2) {}
%       (n3.b) -- +(0mm,5mm) node[above] {$i_5$}
%       (n3.a) |- ++(-5mm,2mm)
%       coordinate (p) -- +(0mm,5mm) node[above] {$i_4$}
%       (n2.c) |- (p)
%       (n2.b) |- ++(6mm,12mm) -- +(0mm,5mm) node[above] {$i_3$}
%       (n2.a) -- +(0mm,8mm)
%       node[and2,anchor=tip,draw] (n1) {}
%       (n1.b) -- +(0mm,5mm) node[above] {$i_2$}
%       (n1.a) -- +(0mm,5mm) node[above] {$i_1$};
% \end{tikzpicture}
% \end{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\pgfsetcktbaselength#1{\def\cktbaselength{#1}}
\pgfsetcktbaselength{2pt}
\tikzoption{cktbaselength}{\pgfsetcktbaselength{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cktsetbasexandyvec{%
\pgfsetxvec{\pgfpoint{\baselength}{0pt}}
\pgfsetyvec{\pgfpoint{0pt}{\baselength}}
}

\def\cktsetcktbasexandyvec{%
\pgfsetxvec{\pgfpoint{\cktbaselength}{0pt}}
\pgfsetyvec{\pgfpoint{0pt}{\cktbaselength}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cktdrawtrianglenonclosed{%
\pgfpathmoveto{\pgfpointorigin}
\pgfpathlineto{\pgfpointxy{10}{20}}
\pgfpathlineto{\pgfpointxy{-10}{20}}
}

\def\cktdrawfitwotrunk{%
\pgfpathmoveto{\pgfpointxy{20}{28}}
\pgfpathcurveto{\pgfpointxy{20}{4}}{\pgfpointxy{8}{0}}{\pgfpointorigin}
\pgfpathcurveto{\pgfpointxy{-8}{0}}{\pgfpointxy{-20}{4}}{\pgfpointxy{-20}{28}}
}

\def\cktdrawandtwoshape{%
\cktdrawfitwotrunk
\pgfpathclose
}

\def\cktdrawortwoshape{%
\cktdrawfitwotrunk
\pgfpathcurveto{\pgfpointxy{-6}{16}}{\pgfpointxy{6}{16}}{\pgfpointxy{20}{28}}
\pgfpathclose
}

\def\cktdrawfithreetrunk{%
\pgfpathmoveto{\pgfpointxy{30}{30}}
\pgfpathcurveto{\pgfpointxy{30}{6}}{\pgfpointxy{12}{0}}{\pgfpointorigin}
\pgfpathcurveto{\pgfpointxy{-12}{0}}{\pgfpointxy{-30}{6}}{\pgfpointxy{-30}{30}}
}

\def\cktdrawandthreeshape{%
\cktdrawfithreetrunk
\pgfpathclose
}

\def\cktdraworthreeshape{%
\cktdrawfithreetrunk
\pgfpathcurveto{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}
\pgfpathclose
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cktlocateortwoaanchor{%
\pgfpointcurveattime{0.2452}{\pgfpointxy{-20}{28}}{\pgfpointxy{-6}{16}}{\pgfpointxy{6}{16}}{\pgfpointxy{20}{28}}%
}

\def\cktlocateorthreeaanchor{%
\pgfpointcurveattime{0.1667}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
}

\def\cktlocateorthreebanchor{%
\pgfpointcurveattime{0.5}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cktdrawzinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{0}{-3}}{3\@tempdima}
}

\def\cktdrawandtwoainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{-10}{31}}{3\@tempdima}
}

\def\cktdrawandtwobinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{10}{31}}{3\@tempdima}
}

\def\cktdrawortwoainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{-10\@tempdima}{\ycirccenter}}{3\@tempdima}
}

\def\cktdrawortwobinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{10\@tempdima}{\ycirccenter}}{3\@tempdima}
}

\def\cktdrawandthreeainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{-20}{33}}{3\@tempdima}
}

\def\cktdrawandthreebinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{0}{33}}{3\@tempdima}
}

\def\cktdrawandthreecinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{20}{33}}{3\@tempdima}
}

\def\cktdraworthreeainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{-20\@tempdima}{\ycirccenter}}{3\@tempdima}
}

\def\cktdraworthreebinversion{%
\pgfpointcurveattime{0.5}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
\@tempdima=\baselength
\advance\pgf@y by 3\@tempdima
\pgfpathcircle{\pgfpoint{\pgf@x}{\pgf@y}}{3\@tempdima}
}

\def\cktdraworthreecinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{20\@tempdima}{\ycirccenter}}{3\@tempdima}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{buffer}{
  \saveddimen{\baselength}{
    \pgf@x=\cktbaselength
  }
  % TODO: chose barycenter for center instead?
  \anchor{center}{     \cktsetbasexandyvec \pgfpointxy{0}{10} }
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-10}{20} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{20} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{10}{20} }
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-10}{10} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{10}{10} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-10}{0} }
  \anchor{south}{      \pgfpointorigin }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{10}{0} }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{0}{20} }
  \anchor{z}{          \pgfpointorigin }
  \anchor{tip}{        \pgfpointorigin }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawtrianglenonclosed
    \pgfpathclose
  }
}

\pgfdeclareshape{inverter}{
  \inheritsavedanchors[from=buffer]
  \inheritanchor[from=buffer]{center}
  \inheritanchor[from=buffer]{north west}
  \inheritanchor[from=buffer]{north}
  \inheritanchor[from=buffer]{north east}
  \inheritanchor[from=buffer]{tip}
  \inheritanchor[from=buffer]{a}
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-10}{7} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{10}{7} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-10}{-6} }
  \anchor{south}{      \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{10}{-6} }
  \anchor{z}{          \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \backgroundpath{
    \cktsetbasexandyvec
    % The inverter looks nicer if the path is not closed.
    \cktdrawtrianglenonclosed
    \pgfpathlineto{\pgfpointorigin}
    \cktdrawzinversion
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{and2}{
  \saveddimen{\baselength}{
    \pgf@x=\cktbaselength
  }
  % TODO: chose barycenter for center instead?
  \anchor{center}{     \cktsetbasexandyvec \pgfpointxy{0}{14} }
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{28} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{28} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{28} }
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-20}{14} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{20}{14} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-20}{0} }
  \anchor{south}{      \pgfpointorigin }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{20}{0} }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{-10}{28} }
  \anchor{b}{          \cktsetbasexandyvec \pgfpointxy{10}{28} }
  \anchor{z}{          \pgfpointorigin }
  \anchor{tip}{        \pgfpointorigin }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
  }
}

\pgfdeclareshape{nand2ii}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{west}
  \inheritanchor[from=and2]{east}
  \inheritanchor[from=and2]{tip}
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{34} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{34} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{34} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-20}{-6} }
  \anchor{south}{      \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{20}{-6} }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{-10}{34} }
  \anchor{b}{          \cktsetbasexandyvec \pgfpointxy{10}{34} }
  \anchor{z}{          \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwoainversion
    \cktdrawandtwobinversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{and2in}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2ii]{north west}
  \inheritanchor[from=nand2ii]{north}
  \inheritanchor[from=nand2ii]{north east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=nand2ii]{a}
  \inheritanchor[from=and2]{b}
  \inheritanchor[from=and2]{z}
  \inheritanchor[from=and2]{tip}
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-20}{17} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{20}{17} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwoainversion
  }
}

\pgfdeclareshape{and2ni}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2ii]{north west}
  \inheritanchor[from=nand2ii]{north}
  \inheritanchor[from=nand2ii]{north east}
  \inheritanchor[from=and2in]{west}
  \inheritanchor[from=and2in]{east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=and2]{a}
  \inheritanchor[from=nand2ii]{b}
  \inheritanchor[from=and2]{z}
  \inheritanchor[from=and2]{tip}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwobinversion
  }
}

\pgfdeclareshape{and2ii}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2ii]{north west}
  \inheritanchor[from=nand2ii]{north}
  \inheritanchor[from=nand2ii]{north east}
  \inheritanchor[from=and2in]{west}
  \inheritanchor[from=and2in]{east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=nand2ii]{a}
  \inheritanchor[from=nand2ii]{b}
  \inheritanchor[from=and2]{z}
  \inheritanchor[from=and2]{tip}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwoainversion
    \cktdrawandtwobinversion
  }
}

\pgfdeclareshape{nand2}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{north west}
  \inheritanchor[from=and2]{north}
  \inheritanchor[from=and2]{north east}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{a}
  \inheritanchor[from=and2]{b}
  \inheritanchor[from=nand2ii]{z}
  \inheritanchor[from=and2]{tip}
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-20}{11} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{20}{11} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawzinversion
  }
}

\pgfdeclareshape{nand2in}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2ii]{north west}
  \inheritanchor[from=nand2ii]{north}
  \inheritanchor[from=nand2ii]{north east}
  \inheritanchor[from=nand2ii]{west}
  \inheritanchor[from=nand2ii]{east}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=nand2ii]{a}
  \inheritanchor[from=and2]{b}
  \inheritanchor[from=nand2ii]{z}
  \inheritanchor[from=and2]{tip}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwoainversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{nand2ni}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2ii]{north west}
  \inheritanchor[from=nand2ii]{north}
  \inheritanchor[from=nand2ii]{north east}
  \inheritanchor[from=nand2ii]{west}
  \inheritanchor[from=nand2ii]{east}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{a}
  \inheritanchor[from=nand2ii]{b}
  \inheritanchor[from=nand2ii]{z}
  \inheritanchor[from=and2]{tip}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandtwoshape
    \cktdrawandtwobinversion
    \cktdrawzinversion
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{or2}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{north west}
  \inheritanchor[from=and2]{north}
  \inheritanchor[from=and2]{north east}
  \inheritanchor[from=and2]{west}
  \inheritanchor[from=and2]{east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=and2]{z}
  \anchor{a}{ \cktsetbasexandyvec \cktlocateortwoaanchor }
  \anchor{b}{ \cktsetbasexandyvec \cktlocateortwoaanchor \pgf@x=-\pgf@x }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
  }
}

\pgfdeclareshape{nor2ii}{
  \inheritsavedanchors[from=and2]
  \saveddimen\ycirccenter{
    \cktsetcktbasexandyvec
    \pgfpointxy{24.685}{0}
  }
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nand2]{west} % TODO: This is not exact
  \inheritanchor[from=nand2]{east} % TODO: This is not exact
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nand2ii]{z}
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{3} \advance\pgf@y by \ycirccenter }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{3} \advance\pgf@y by \ycirccenter }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{3} \advance\pgf@y by \ycirccenter }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{-10}{3} \advance\pgf@y by \ycirccenter }
  \anchor{b}{          \cktsetbasexandyvec \pgfpointxy{10}{3} \advance\pgf@y by \ycirccenter }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwoainversion
    \cktdrawortwobinversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{or2in}{
  \inheritsavedanchors[from=nor2ii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor2ii]{north west}
  \inheritanchor[from=nor2ii]{north}
  \inheritanchor[from=nor2ii]{north east}
  \inheritanchor[from=nand2ii]{east} % TODO: This is not exact
  \inheritanchor[from=nand2ii]{west} % TODO: This is not exact
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nor2ii]{a}
  \inheritanchor[from=or2]{b}
  \inheritanchor[from=and2]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwoainversion
  }
}

\pgfdeclareshape{or2ni}{
  \inheritsavedanchors[from=nor2ii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor2ii]{north west}
  \inheritanchor[from=nor2ii]{north}
  \inheritanchor[from=nor2ii]{north east}
  \inheritanchor[from=or2in]{west}
  \inheritanchor[from=or2in]{east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=or2]{a}
  \inheritanchor[from=nor2ii]{b}
  \inheritanchor[from=and2]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwobinversion
  }
}

\pgfdeclareshape{or2ii}{
  \inheritsavedanchors[from=nor2ii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor2ii]{north west}
  \inheritanchor[from=nor2ii]{north}
  \inheritanchor[from=nor2ii]{north east}
  \inheritanchor[from=or2in]{west}
  \inheritanchor[from=or2in]{east}
  \inheritanchor[from=and2]{south east}
  \inheritanchor[from=and2]{south}
  \inheritanchor[from=and2]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nor2ii]{a}
  \inheritanchor[from=nor2ii]{b}
  \inheritanchor[from=and2]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwoainversion
    \cktdrawortwobinversion
  }
}

\pgfdeclareshape{nor2}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{north west}
  \inheritanchor[from=and2]{north}
  \inheritanchor[from=and2]{north east}
  \inheritanchor[from=nand2]{east}
  \inheritanchor[from=nand2]{west}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=or2]{a}
  \inheritanchor[from=or2]{b}
  \inheritanchor[from=nor2ii]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawzinversion
  }
}

\pgfdeclareshape{nor2in}{
  \inheritsavedanchors[from=nor2ii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor2ii]{north west}
  \inheritanchor[from=nor2ii]{north}
  \inheritanchor[from=nor2ii]{north east}
  \inheritanchor[from=nor2ii]{west}
  \inheritanchor[from=nor2ii]{east}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nor2ii]{a}
  \inheritanchor[from=or2]{b}
  \inheritanchor[from=nor2ii]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwoainversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{nor2ni}{
  \inheritsavedanchors[from=nor2ii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor2ii]{north west}
  \inheritanchor[from=nor2ii]{north}
  \inheritanchor[from=nor2ii]{north east}
  \inheritanchor[from=nor2ii]{west}
  \inheritanchor[from=nor2ii]{east}
  \inheritanchor[from=nand2ii]{south east}
  \inheritanchor[from=nand2ii]{south}
  \inheritanchor[from=nand2ii]{south west}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=or2]{a}
  \inheritanchor[from=nor2ii]{b}
  \inheritanchor[from=nor2ii]{z}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawortwoshape
    \cktdrawortwobinversion
    \cktdrawzinversion
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfdeclareshape{and3}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=and2]{z}
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{30} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30} }
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-30}{15} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{30}{15} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{0} }
  \anchor{south}{      \pgfpointorigin }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{0} }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{-20}{30} }
  \anchor{b}{          \cktsetbasexandyvec \pgfpointxy{0}{30} }
  \anchor{c}{          \cktsetbasexandyvec \pgfpointxy{20}{30} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandthreeshape
  }
}

\pgfdeclareshape{nand3iii}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nand2ii]{z}
  \inheritanchor[from=and3]{west}
  \inheritanchor[from=and3]{east}
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{36} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{36} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{36} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{-6} }
  \anchor{south}{      \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{-6} }
  \anchor{a}{          \cktsetbasexandyvec \pgfpointxy{-20}{36} }
  \anchor{b}{          \cktsetbasexandyvec \pgfpointxy{0}{36} }
  \anchor{c}{          \cktsetbasexandyvec \pgfpointxy{20}{36} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandthreeshape
    \cktdrawandthreeainversion
    \cktdrawandthreebinversion
    \cktdrawandthreecinversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{and3nni}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=and2]{z}
  \inheritanchor[from=nand3iii]{north west}
  \inheritanchor[from=nand3iii]{north}
  \inheritanchor[from=nand3iii]{north east}
  \inheritanchor[from=and3]{south west}
  \inheritanchor[from=and3]{south}
  \inheritanchor[from=and3]{south east}
  \inheritanchor[from=and3]{a}
  \inheritanchor[from=and3]{b}
  \inheritanchor[from=nand3iii]{c}
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-30}{18} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{30}{18} }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdrawandthreeshape
    \cktdrawandthreecinversion
  }
}

\pgfdeclareshape{or3}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=and2]{z}
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{30} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30} }
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-30}{15} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{30}{15} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{0} }
  \anchor{south}{      \pgfpointorigin }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{0} }
  \anchor{a}{ \cktsetbasexandyvec \cktlocateorthreeaanchor }
  \anchor{b}{ \cktsetbasexandyvec \cktlocateorthreebanchor }
  \anchor{c}{ \cktsetbasexandyvec \cktlocateorthreeaanchor \pgf@x=-\pgf@x }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdraworthreeshape
  }
}

\pgfdeclareshape{nor3iii}{
  \inheritsavedanchors[from=and2]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=nand2ii]{z}
  \saveddimen\ycirccenter{
    \cktsetcktbasexandyvec
    \pgfpointxy{27.505}{0}
  }
  \anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30.505} }
  \anchor{north}{      \cktsetbasexandyvec \pgfpointxy{0}{30.505} }
  \anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30.505} }
  \anchor{west}{       \cktsetbasexandyvec \pgfpointxy{-30}{15.2525} }
  \anchor{east}{       \cktsetbasexandyvec \pgfpointxy{30}{15.2525} }
  \anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{-6} }
  \anchor{south}{      \cktsetbasexandyvec \pgfpointxy{0}{-6} }
  \anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{-6} }
  \anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-20}{3} \advance\pgf@y by \ycirccenter }
  \anchor{b}{
    \cktsetbasexandyvec
    \pgfpointcurveattime{0.5}%
        {\pgfpointxy{-30}{30}}%
        {\pgfpointxy{-10}{16}}%
        {\pgfpointxy{10}{16}}%
        {\pgfpointxy{30}{30}}%
    \@tempdima=\baselength
    \advance\pgf@y by 6\@tempdima
  }
  \anchor{c}{ \cktsetbasexandyvec \pgfpointxy{20}{3} \advance\pgf@y by \ycirccenter }
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdraworthreeshape
    \cktdraworthreeainversion
    \cktdraworthreebinversion
    \cktdraworthreecinversion
    \cktdrawzinversion
  }
}

\pgfdeclareshape{or3nni}{
  \inheritsavedanchors[from=nor3iii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=nor3iii]{north west}
  \inheritanchor[from=nor3iii]{north}
  \inheritanchor[from=nor3iii]{north east}
  \inheritanchor[from=or3]{east} % TODO: This is not exact
  \inheritanchor[from=or3]{west} % TODO: This is not exact
  \inheritanchor[from=or3]{south west}
  \inheritanchor[from=or3]{south}
  \inheritanchor[from=or3]{south east}
  \inheritanchor[from=and2]{tip}
  \inheritanchor[from=and2]{z}
  \inheritanchor[from=or3]{a}
  \inheritanchor[from=or3]{b}
  \inheritanchor[from=nor3iii]{c}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdraworthreeshape
    \cktdraworthreecinversion
  }
}

\pgfdeclareshape{nor3}{
  \inheritsavedanchors[from=nor3iii]
  \inheritanchor[from=and2]{center}
  \inheritanchor[from=or3]{north west}
  \inheritanchor[from=or3]{north}
  \inheritanchor[from=or3]{north east}
  \inheritanchor[from=or3]{east} % TODO: This is not exact
  \inheritanchor[from=or3]{west} % TODO: This is not exact
  \inheritanchor[from=nor3iii]{south west}
  \inheritanchor[from=nor3iii]{south}
  \inheritanchor[from=nor3iii]{south east}
  \inheritanchor[from=nand2ii]{tip}
  \inheritanchor[from=nand2ii]{z}
  \inheritanchor[from=or3]{a}
  \inheritanchor[from=or3]{b}
  \inheritanchor[from=or3]{c}
  \backgroundpath{
    \cktsetbasexandyvec
    \cktdraworthreeshape
    \cktdrawzinversion
  }
}


